Conceptual design of the Spin Physics Detector

The Spin Physics Detector, a universal facility for studying the nucleon spin structure and other spin-related phenomena with polarized proton and deuteron beams, is proposed to be placed in one of the two interaction points of the NICA collider that is under construction at the Joint Institute for Nuclear Research (Dubna, Russia). At the heart of the project there is huge experience with polarized beams at JINR. The main objective of the proposed experiment is the comprehensive study of the unpolarized and polarized gluon content of the nucleon. Spin measurements at the Spin Physics Detector at the NICA collider have bright perspectives to make a unique contribution and challenge our understanding of the spin structure of the nucleon. In this document the Conceptual Design of the Spin Physics Detector is presented.

==> Makefile <==
MAINFILE=SPD_CDR
TEXFILES=$(wildcard *.tex) \
         $(wildcard ./*/*.tex) \
         $(wildcard ./*/*/*.tex)
INCFILES=$(wildcard *.tex)
AUXFILES=$(patsubst %.tex, %.aux, $(INCFILES)) 
#AUXFILES=$(wildcard *.aux)
BIBFILES=$(wildcard ./bib/*.bib)
BBLFILES=$(patsubst %.tex, %.bbl, $(INCFILES)) 
#BBLFILES=$(MAINFILE).bbl
FIGFILES=$(wildcard ./fig/*.pdf) \
         $(wildcard ./fig/*.jpg) \
         $(wildcard ./fig/*.png) 

export TEXINPUTS=.:./sty:./tex:./bib:$TEXINPUTS:
export BSTINPUTS=.:./sty:$BSTINPUTS:
export BIBINPUTS=.:./bib:$BIBINPUTS:

all:	$(MAINFILE).pdf

test:
	@echo ``TEXFILES:'' $(TEXFILES)
	@echo ``INCFILES:'' $(INCFILES)
	@echo ``AUXFILES:'' $(AUXFILES)
	@echo ``BIBFILES:'' $(BIBFILES)
	@echo ``BBLFILES:'' $(BBLFILES)
	@echo ``FIGFILES:'' $(FIGFILES)

emacs:
	emacs $(TEXFILES) &

$(MAINFILE).pdf: $(MAINFILE).tex $(FIGFILES) $(TEXFILES) $(BBLFILES)
	@echo "============ Main LaTeX pass ============"
	-pdflatex --shell-escape $(MAINFILE) 
	pdflatex --shell-escape $(MAINFILE) 
#	pdflatex --shell-escape $(MAINFILE) 

%.bbl:	%.aux 
	@echo "============ BibTeX pass ============"
	-bibtex $(patsubst %.aux,%,$^)

#%.bbl: %.tex $(BIBFILES)
#	-bibtex $(MAINFILE)

%.aux: 	%.tex
	@echo "============ TEX -> AUX pass for" $@ "============" 
	-pdflatex --shell-escape $(MAINFILE) 

clean:
	@echo "============ Cleaning ============" 
	-rm -rf *.aux *.blg *.bbl *.log *.out *.toc *.lof *.brf

distclean: clean
	@echo "============ Thorough cleaning ============" 
	-rm -rf $(MAINFILE).pdf *~

.PRECIOUS: %.bbl %.aux

.PHONY: clean distclean test all emacs



==> fig/conclusion.tex <==
\chapter{Conclusion}
The proposed physics program and the concept of the SPD facility presented in the document, are open for exciting and challenging ideas from theorists and experimentalists worldwide.  The Conceptual Design Report of the Spin Physics Detector was presented and discussed at the 54th meeting of the JINR Program Advisory Committee for Particle Physics on January 18, 2021. The following recommendations were obtained: 
{\it 
      The PAC thanks the SPD (proto-)collaboration for the preparation of the comprehensive CDR and recommends the NICA management to appoint an appropriate Detector Advisory Committee for a thorough review of the CDR and its subsequent evolution into an SPD TDR (Technical Design Report). The PAC encourages the team to pursue every effort to form an international collaboration, find adequate resources and attract students and young scientists.
}

The international Detector Advisory Committee (SPD DAC) was formed in April 2021. 
The Committee is chaired by A. Bressan (University of Trieste, Italy) and includes P. Di Nezza (National Institute for Nuclear Physics, Frascati, Italy) and a member of the PAC P. Hristov (CERN, Switzerland). The report was presented by A. Bressan on behalf of the SPD DAC at the 56th meeting of the JINR Program Advisory Committee for Particle Physics on January 24, 2022. As an outcome of the report, the PAC issued the following recommendations:

{\it 
The PAC notes with interest the evaluation report presented by A. Bressan on behalf of the SPD DAC. The Committee held several meetings with the SPD team and asked several questions concerning the SPD detector concept. In addition to that, issues related to the NICA complex infrastructure for polarized beams and possible interactions between the SPD and MPD experiments were discussed in depth. The answers to the DAC's questions were satisfactory and the presentations during the joint meetings were well received by the committee. The DAC particularly appreciated the improvements in the SPD conceptual design with respect to the original CDR, namely changing the magnet location to be outside the ECAL, the possible use of a full MAPS inner tracker, and the clarifications on the straw detectors and the ZDC. On the basis of all that, and following the recommendation of the DAC, \textbf{the PAC approves the SPD CDR and asks the SPD team to move forward to the TDR preparation.} The PAC appreciates the important role of the DAC in the SPD project evaluation and requests periodic DAC reports.

}

==> fig/institutions.tex <==
\chapter{Participating institutions and author list}

%Host institute of the project is the Laboratory of High-Energy Physics of the Joint Institute for Nuclear Research. 
%The main part of the human resources engaged with the project comes from there (61 researchers, 24.4 FTE). 
%The Laboratory of Nuclear Problems is the other laboratory of the JINR that participates in the project with substantial number of researchers (29 researchers, 11.3 FTE).
%Altogether the JINR engagement in the project now evaluates to 37.7 full-time-equivalent (FTE) researchers.

%Fourteen institutes from the JINR Member States and other countries have expressed by now their interest for participation 
%in the project and indicate that they could allocate resources and manpower for the project. The list of institutes together 
%with the names of researchers (in some cases only the leaders of the teams are listed) is given below. Received Expressions of Interest are collected under a separate cover.

\begin{center}
{\large \bf National Science Laboratory, Armenia}\\
Akopov N., Movsisyan A.
\end{center}

\begin{center}
{\large \bf Institute of Applied Physics 
of the National Academy of Sciences of Belarus, Minsk, Belarus }\\
Shulyakovsky R.
\end{center}

\begin{center}
{\large \bf Research Institute for Nuclear Problems of Belarusian State University, Minsk, Belarus}\\
Korjik M.V., Lobko A.S., Makarenko V.V., Solin A.A., Solin A.V.
\end{center}

\begin{center}
{\large \bf Universidad Andrés Bello, Santiago, Chile}\\
Kuleshov S., Zamora J.
\end{center}

\begin{center}
{\large \bf China Institute of Atomic Energy, Beijing, China}\\
Chen Lei, Jia Shi-Hai, Li Pei-Yu, Li Xiao-Mei, Song Jin-Xin, Sun Hao, Sun Peng-Fei, Zhang Yun-Yu, Zhang Jun-Wei, Zhao Ming-Rui, Zhi Yu
\end{center}

\begin{center}
{\large \bf Higher Institute of Technologies and Applied Sciences (InSTEC), Havana University, Havana, Cuba }\\
Guzman F., Gars\'{i}a Trapaga C.E. 
\end{center}

\begin{center}
{\large \bf Charles University, Prague, Czech Republic }\\
Finger M., Finger M. (jr.), Prochazka I., Slunecka M., Sluneckova V.
\end{center}

\begin{center}
{\large \bf Czech Technical University in Prague, Czech Republic }\\
Havranek M., Jary V., Lednicky D., Marcisovsky M., Neue G., Popule J., Tomasek L., Virius M., \fbox{Vrba V.}
\end{center}

\begin{center}
{\large \bf University of Turin and INFN Section, Turin, Italy}\\
Alexeev M., Amoroso A., Chiosso M., Denisov O.Yu., Kotzinian A., Maggiora A., Panzieri D., Parsamyan B., Tosello F.
\end{center}

\begin{center}
{\large \bf Warsaw University of Technology, Warsaw, Poland}\\
Buchowicz A., Dygnarowicz K., Galiński G., Klekotko A., Kurjata R., Marzec J., Pastuszak G., Rychter A., Zaremba K., Ziembicki M.
\end{center}


\begin{center}
{\large \bf Joint Institute for Nuclear Research, JINR, Dubna, Russia}\\

%{\bf Directorate}\\

%Lednick\'{y} R. \\

{\bf Laboratory of High-Energy Physics}\\

Akhunzyanov R.R., Alexakhin V.Yu., Anosov V.A.,  Azorskiy N.I., Baldin A.A., Baldina E.G., Barabanov M.Yu., 
%Batozskaya V.S., 
 Beloborodov A.N., Belyaev A. V., Bleko V.V., Bogoslovsky D.N., Boguslavsky I.N.,  Burtsev V.E.,
%Boguslavskiy I.V, 
 Dunin V.B., Enik T.L., Filatov Yu.N.\footnote{also Moscow Institute of Physics and Technology, Dolgoprudny, Russia}, Gavrishchuk O.P., Galoyan A.S., Glonti L., Golubykh S.M., Grafov N.O., Gribovsky A.S., Gromov S.A., Gromov V.A., Gurchin Yu.V., Gusakov Yu.V., Ivanov A.V., Ivanov N.Ya., Isupov A.Yu., Kasianova E.A., Kekelidze G.D., Khabarov S.V., Kharusov P.R., Khrenov A.N.,  Kokoulina E.S., Kopylov Yu.A.,  Korovkin P.S., Korzenev A. Yu., Kostukov  E.V., \fbox{Kovalenko A.D.}, Kozhin M.A., Kramarenko V.A., Kruglov V.N., Ladygin E.A., Ladygin V.P., Lednick\'{y} R., Livanov A.N., Lysan V.M., Makankin A.M., Martovitsky E.V., Meshcheriakov G.V.,  Moshkovsky I.V., Nagorniy S.N., Nikiforov D.N. Nikitin V.A., Parzhitsky S.S., Pavlov V.V.,  Perepelkin E.E.,  Peshekhonov D.V., Popov V.V., Reznikov S.G., Rogachevsky O.V., Safonov A.B., Salamatin K.M., Savenkov A.A.,   Sheremeteva A.I., Shimanskii S.S.,
 %Savin I.A., 
  Starikova S.Yu., Streletskaya E.A., 
 %Strokovsky E.A.,
 Tarasov O.G., Terekhin A.A., Teryaev O.V., Tishevsky A.V., Topilin N.D., Topko B.L., Troyan. Yu.A., Usenko E.A., Vasilieva E.V., Volkov I.S.,Volkov P.V., Yudin I.P., Zamyatin N.I., Zemlyanichkina E.V., Zhukov I.A., Zinin A.V., Zubarev E.V.

{\bf Laboratory of Nuclear Problems} \\

Abazov V.M., Afanasyev L.G., Alexeev G.D., Balandina V.V., Belova A.P., Bobkov A.V., Boltushkin E.V., Brazhnikov E.V., Datta A., Denisenko I.I.,  Duginov V.N., 
%Finger M., Finger M (jr.),
Frolov V.N., Golovanov G.A., Gridin A.O., Gritsay K. I., Guskov A.V., Kirichkov N.V., Komarov V.I., Kulikov A.V., Kurbatov V.S.,  Kutuzov S.A., Maltsev A., Mitrofanov E.O.,  Nefedov Yu.A., Pavlova A.A., Piskun A.A., Prokhorov I.K., Rezvaya E.P.,  Romanov V.M., Rudenko A.I., Rumyantsev M.A., Rybakov N.A., Rymbekova A.,  Samartsev A.G., Shaikovsky V.N., Shtejer K., Sinitsa A.A., Skachkov N.B., Skachkova A.N., 
%Slunecka M., Sluneckova V.,
 Tereschenko V.V., Tkachenko A.V., Tokmenin V.V., Trunov N.O., Uzikov Yu.N., Verkheev A.Yu., Vertogradov L.S., Vertogradova Yu.L., Vesenkov V.A., Zhemchugov A.S., Zhuravlev N.I.

{\bf Laboratory of Theoretical Physics} \\
Anikin I.V., Arbuzov A.B., \fbox{Efremov A.V.}, Goloskokov S.V., Klopot Ya., Strusik-Kotlozh D., Volchansky N.I. 

{\bf Laboratory of Information Technologies} \\
Goncharov P.V., Oleynik D.A., Ososkov G.A., Petrosyan A.Sh., Podgainy D.V., Pelevanyuk I.S., Polyakova R.V., Uzhinsky V.V., Zuev M.I.

\end{center}

\begin{center}
{\large \bf St. Petersburg Nuclear Physics Institute, Gatchina, Russia}\\
Barsov S.G., Fedin O.L., Kim V.T., Kuznetsova E.V., Maleev V.P., Shavrin A.A., Zelenov A.V.
\end{center}

\begin{center}

{\large \bf  Lebedev Physical Institute of the Russian Academy of Sciences, Moscow, Russia}\\

Andreev V.F., Baskov V.A., Dalkarov O.D., Demikhov E.I., Gerasimov S.G., L'vov A.I., Negodaev M.A., Nechaeva P.Yu., Polyansky V.V.,  Suchkov S.I., Terkulov A.R.,  Topchiev N.P.

\end{center}

\begin{center}
{\large \bf  Skobeltsin Institute of Nuclear Physics of the Moscow State University,
Moscow, Russia}\\
Aleshko A.M., Belov I.N., Berezhnoy A.V., Boos E.E., Bunichev V.E., Chepurnov A.S., Gribkov D.Y., Merkin M.M., Nikolaev A.S. 

\end{center}

\begin{center}
{\large \bf  Institute for Theoretical and Experimental Physics, Moscow, Russia}\\
Akindinov A.V.,
Alekseev I.G., 
Golubev A.A.,
Kirin D.Yu.,
Luschevskaya E.,
Malkevich D.B.,
Morozov B.,
Plotnikov V.V.,
Polozov P.,
Rusinov V.,
Stavinskiy A.V.,
Sultanov R.I., 
Svirida D.N.,
Tarkovskyi E.I.,
Zhigareva N.M.
%E. Samigullin (PhD student), Ye. Karkaryan and V. Tyasin (bachelor student)
\end{center}

\begin{center}
{\large \bf  Institute for High-Energy Physics, Protvino, Russia}\\
Vorobiev A.
\end{center}

\begin{center}
{\large \bf Samara National Research University, Samara, Russia}\\
Karpishkov A.V., Nefedov M.A., Saleev V.A., Shipilova  A.V.
\end{center}

\begin{center}
{\large \bf St. Petersburg Polytechnic University, St. Petersburg, Russia}\\
Berdnikov A.Ya., Berdnikov Ya.A., Borisov V.S., Larionova D.M., Mitrankov Yu.M., Mitrankova M.M.
\end{center}

\begin{center}
{\large \bf St. Petersburg State University, St. Petersburg, Russia }\\
Feofilov G.A., Kovalenko V.N., Valiev F.F., Vechernin V.V., Zherebchevsky V.Yo.
\end{center}

\begin{center}
{\large \bf Tomsk State University, Tomsk, Russia }\\
 Chumakov A., Lyubovitskij V., Trifonov A.,  Zhevlakov A. 
\end{center}

\begin{center}
{\large \bf Belgorod State University, Belgorod, Russia }\\
Kaplii A.,
Kishchin I.,
Kluev A.,
Kubankin A., 
Kubankin Yu.
\end{center}

\begin{center}
{\large \bf University of Belgrade, Institute of Physics Belgrade, Belgrade, Serbia}\\
Jokovic D., Maletic D., Savic M.
\end{center}             
                
\begin{center}
{\large \bf V.N. Karazin Kharkiv National University,  Kharkiv, Ukraine}\\
Kovtun V.E., Lyashchenko V.N., Malykhina T.V., Reva S.N., Sotnikov V.V.
\end{center}              

\begin{center}
{\large \bf Institute for Scintillation Materials National Academy of Sciences of Ukraine (Kharkiv, Ukraine)}\\
Boyarintsev A.Yu., Eliseev D.A., Grinyov B.V., Zhmurin P.N.
\end{center}           


                
\begin{center}
{\large \bf Individual contributors:}\\
Abramov V. (IHEP, Russia), El-Kholy R. (Cairo University), Haidenbauer J. (IAS and IKP, Forschungszentrum J{\"u}lich), 
Kondratenko A.M. (STL ''Zaryad'', Novosibirsk, Russia and Moscow Institute of Physics and Technology, Dolgoprudny, Russia),
Kondratenko M.A. (STL ''Zaryad'', Novosibirsk, Russia and Moscow Institute of Physics and Technology, Dolgoprudny, Russia),
Konorov I. (Technical University of Munich), Richard J.-M. (Universit\'e de Lyon), Semak A.A. (Institute of High Energy Physics, Protvino, Russia) Strikman M. (Penn State University),    Temerbayev  A. ( L.N. Gumilyov Eurasian National University, Nur-Sultan), Tomasi-Gustafsson E. (DPhN, IRFU, CEA, Universit\'e Paris-Saclay),  
Tsenov R. (University of Sofia), Wang Q. (South China Normal University, Guangzhou), Zhao Q. (Institute of High Energy Physics, CAS, Beijing)
\end{center}

\begin{center}
We are also grateful to  Kukhtin V. V., Nagaytsev A.P.,  Savin I.A., \fbox{Shevchenko O. Yu.}, and \fbox{Sisakyan A.N.} for their invaluable contribution to the SPD project at earlier stages of its implementation.
\end{center}

\begin{center}
{\large \bf
Acknowledgements.\\}
This work is supported by the RFBR research projects No. 18-02-40097 and 18-02-40061.
\end{center}

% Prof. Adam Kisiel,
% Warsaw University of Technology, Warsaw, Poland		                               kisiel@if.pw.edu.pl 

% Prof. Tomasz Starecki,
% Warsaw University of Technology, Warsaw, Poland		                        t.starecki@eka.pw.edu.pl

% Prof. Krzysztof Kurek
% National Centre for Nuclear Research, Swierk, Poland                       krzysztof.kurek@ncbj.gov.pl 

% Prof. Yury Kryshnev,
% % Gomel State Technical University, Gomel, Belarus    				 kaf_pe@gstu.by 


% Dr. Nikolai Nikolaev,
% Landau institute for Theoretical Physics, Moscow, Russia			        nikolaev@itp.ac.ru

%ИСМА НАНУ, Харьков (адрес и пр. - на сайте)
%Institute for Scintillation Materials National Academy of Sciences of Ukraine (ISMA NANU)

%1. Grinyov B.V.
%2. Boyarintsev A.Yu.
%3. Zhmurin P.N.
%4. Eliseev D.A.



==> tex/DAQ1.tex <==
\chapter{Data acquisition system}
\chapter{Slow control system}

==> tex/PP_MC.tex <==
\subsection{Physics with prompt photons}
\subsubsection{Signal and backgrounds}
Gluon Compton scattering (GCS) is the main mechanism of the prompt-photon production at SPD energies. At $\sqrt{s}=26$ GeV the corresponding cross section calculated in the leading order is 1.2 $\mu$b. Contribution of the competitive quark-antiquark annihilation process is one order of magnitude smaller. Nevertheless the main source of photons in hadronic collisions is the decay of secondary particles, mainly $2\gamma$ decay of $\pi^0$ and $\eta$ mesons. Contributions of  photons from decays of  different secondary particles  per one interaction are presented in Tab. \ref{tab:gamma_bkg}. The $p_T$ spectra of the GCS photons and the decay photons produced near the interaction point are shown in Fig. \ref{fig:pp_rec1}. Contribution of the decay photons dominates over GCS signal in full range of $p_T$ but relative fraction of signal photons  increases with increasing $p_T$. The rejection of photons from reconstructed 2$\gamma$ decays of $\pi^0$ and $\eta$-mesons and the following Monte Carlo-based statistical subtraction of residual background photons is only a way to access the prompt-photon production cross-section at high $p_T$.

One more important source of background photons is interaction of secondary particles with material of the setup elements.
Misidentification of charged energy clusters as neutral in the ECAL due to inefficiency of track finding and reconstruction algorithms produces additional contribution to the background rate. Overlapping of clusters produced by different particles could also contribute to background via distortion of reconstructed kinematics.

\begin{table}[htp]
\caption{Contributions of  photons from decays of  different secondary particles (per one inelastic interaction). }
\begin{center}
\begin{tabular}{|c|c|}
\hline
Decay  & Number of photons \\
\hline
$\pi^0$ & 8.70 \\
$\eta$  & 0.40 \\
$\omega$ & 0.06 \\
$\eta'$  &  0.05 \\
$\Sigma^0$ & 0.04 \\
Others    &  0.01 \\
\hline
\end{tabular}
\end{center}
\label{tab:gamma_bkg}
\end{table}%

\subsubsection{Requirements to performance of the SPD setup}
For successful realisation of the prompt-photon programme the SPD setup and the ECAL have to meet the next requirements:
\begin{itemize}
\item inner space  of the SPD setup should contain as minimal amount of material as possible in order to keep high transparency of the setup for photons;
\item minimal tracking capability should be provided in order to distinguish between charged and neutral clusters in ECAL;
\item reasonable granularity of the ECAL in order to avoid the pile-up effect that reduces the photon reconstruction efficiency 
and distorts kinematics of reconstructed photons;
\item ability to  detect  with reasonable resolution an energy deposit down to 100 MeV to keep high reconstruction efficiency for photons.  It is important to note that this threshold is significantly below the MIP signal ($\sim$ 200~MeV). Figure \ref{fig:pp_rec1}(b) shows the efficiency of the $\pi^0\to\gamma\gamma$ decay reconstruction for different cluster energy thresholds and different granularities of the ECAL.
\end{itemize}

\begin{figure}[!t]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{PP_Pt} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{PP_eff} \\ (b)}
  \end{minipage}
  \caption{ (a) The $p_T$ spectra of GCS prompt photons (red) and photons produced from $\pi^0$ decay (blue). (b) The efficiency of the $\pi^0\to\gamma\gamma$ decay reconstruction in the case when at least one photon has $p_T>2$ GeV/$c$ as a function of cluster energy threshold for different granularities R of the ECAL.}
  \label{fig:pp_rec1}  
\end{figure}

The invariant mass spectrum of two photons reconstructed in the ECAL with 100 MeV and 200 MeV  energy threshold is shown in Fig. \ref{fig:pp_rec2}(a). Relative energy resolution of the ECAL was assumed to be as mentioned in Eq. \ref{eq:ECAL:res}. Gaussian width of the $\pi^0$ peak is 4.6 MeV/$c^2$ and 3.15 MeV/$c^2$ for 100 MeV and 500 MeV thresholds, respectively.

\begin{figure}[!b]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{PP_mass} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{xF_pT} \\ (b)}
  \end{minipage}
  \caption{ (a) The invariant mass spectrum of two photons for two ECAL thresholds: 100 MeV (yellow) and 500 MeV (green). (b) $p_T$ distribution for GCS photons vs. $x_F$.}
  \label{fig:pp_rec2}  
\end{figure}

\subsubsection{Expected accuracy for asymmetries  $A_N$ and $A_{LL}$}

Accuracy of the prompt-photon production cross-section and asymmetries $A_N$ and $A_{LL}$ in p-p collisions is estimated basing on the following assumptions. Data sample corresponds to $10^{7}$ s of data taking (about 100 days) with average luminosity $L=10^{32}~s^{-1}cm^{-2}$. Inefficiency of the photon reconstruction is caused only by geometrical acceptance and material distribution, no threshold for photon reconstruction in the ECAL. LO calculations are used for the GCS cross-section. Only the $\pi^0\to \gamma\gamma$ decay is taken into account as the background. Average $\pi^0$ reconstruction efficiency is 74.9\%. Relative accuracy for the Monte Carlo description of photon reconstruction is 1\%. Two subsamples with equal statistics are collected with each combination of spin orientations.  Absolute polarization of the beam is assumed to be exactly equal to 100\%.

Since low-$p_T$ region is useless for any studies of prompt photons due to huge background while at high-$p_T$ the statistics is very limited, a reasonable cut on transverse momentum of photon has to be applied in order to maximize the accuracy of the planned measurements. For the running conditions mentioned above the optimal value lies at about 5 to 6 GeV/$c$. The total amount of the detected GCS photons with $p_T>5$ GeV/$c$ is expected to be about $6\times10^6$. 

\begin{figure}[!t]
    \center{\includegraphics[width=1\linewidth]{PP_AA}}
  \caption{ Expected accuracy of $A_{N}$ and $A_{LL}$ measurement as function of $x_{F}$.}
  \label{fig:pp_rec3}  
\end{figure}

Figure \ref{fig:pp_rec2}(b) shows $p_T$ distribution for GCS photons vs. $x_F$. Expected accuracy of $A_N$ and $A_{LL}$ measurement in each of four intervals in $x_F$ in the range from -0.89 to 0.89 is shown in Fig \ref{fig:pp_rec3}.  


==> tex/case.tex <==
\section{Physics case}
\input{case_gen}
\input{case_DY}
\input{case_PP}
\input{jpsi}
\input{high_pt}
\subsection{Multi-quark states}
\input{nica_gpds11}
\subsection{Semi-inclusive and exclusive reactions}




==> tex/case_DY.tex <==
\subsection{MMT-DY pair production}
Parton Distribution Functions (PDFs) describe the structure of the nucleon as
a function of the nucleon momentum fraction carried by a parton.
They have been generalized to contain information not only on the longitudinal but also on the 
transverse distributions of partons in a fast moving hadron. 
The recently developed theoretical framework of  ''3-dimensional picture'' of the nucleon 
which also called as ''nucleon tomography''.
In additional of this framework, the effects of intrinsic transverse parton momenta 
are began to be studied which can be described via Transverse-Momentum-Dependent PDFs (TMDs).
These effects are experimentally investigated in Drell-Yan (DY) processes.
From the measured azimuthal asymmetries in unpolarised and polarised DY processes 
a set of PDFs can be derived. 
Eight independent transverse momentum dependent (TMD) parton distributions
were identified at leading twist, with the transverse momentum $k_T$ 
of partons included. The interaction between the active parton in the hadron
and the target spectators leads to the gauge-invariant TMDs. 

\begin{figure}[h]
\begin{center}
\hskip -1cm
\includegraphics[scale=0.4]{chapter1-ris1}
\caption{Leading twist TMD distribution functions. 
The U,L,T correspond to unpolarized, longitudinally polarized and transversely 
polarized nucleons (rows) and quarks (columns).}
\end{center}
\end{figure}

These effects can be experimentally investigated in Drell-Yan (DY) processes.
From the measured azimuthal asymmetries in unpolarised and polarised DY processes 
a set of PDFs can be derived. 

\begin{enumerate}
\item Transversity:  $A_{UT}^{\sin(\phi+\phi_S)}$, 
correlation between quarks the transverse polarization of nucleon;
\item Sivers: $A_{UT}^{\sin(\phi-\phi_S)}$,
correlation the transverse momentum of non-polarized quark with nucleon transverse
polarization;
\item Pretzelosity:  $A_{UT}^{\sin(3\phi-\phi_S)}$,
distribution of the transverse momentum of quarks in the transversely 
polarized nucleon;
\item Boer-Mulders: $A_{UU}^{\cos(2\phi_h)}$,
distribution of the quark transverse momentum in the non-polarized nucleon;
\item Worm-Gears:  $A_{UL}^{\cos(2\phi_h)}$,
correlation between the longitudinal polarization of the nucleon (longitudinal spin)
and the transverse momentum of quarks.
\end{enumerate}
At the sub-leading twist (twist-3), there are still 16 TMD PDFs 
containing the information on the nucleon structure. 
They have no definite physics interpretation yet.
Above mentioned PDFs are proposed to be measured with 
Spin Purpose Detector (SPD)\cite{Savin:2014sva}. 

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.1]{chapter1-ris2}
\caption{Estimated Sivers asymmetries for NICA conditions.$s=400 GeV^2$, $Q^2=4 Gev^2$ (left panel).
$s=400 GeV^2$, $Q^2=15 GeV^2$ (right panel).
Fits for Sivers functions are taken from \cite{Collins:2005ie} (details are given in text).}
\label{fig:theor-sivers}
\end{center}
\end{figure}

Two approaches (methods) are proposed to be used for DY studies
(see section 2 of \cite{Savin:2014sva}).The first one  is the PDFs 
studies via Fourier analysis  to the measured asymmetries \cite{Arnold:2008kf, Gamberg:2006ru, Bacchetta:2008xw, Anselmino:2013rya, Boer:2011xd, Mulders:1995dh, Bacchetta:2006tn},
and second one is the extractions of PDFs via integrated/weighted asymmetries
\cite{Sissakian:2007dv, Sissakian:2005vd, Sissakian:2005yp, Sissakian:2008th, Sissakian:2010zza}. 
For example, the theoretical estimations on Sivers asymmetries 
are given in Figure\ref{fig:theor-sivers}.
Three different fitting functions for the Sivers distributions
are used to estimate asymmetries in Figure \ref{fig:theor-sivers}:
fits I and II from  \cite{Efremov:2005} and the last fit
from \cite{Collins:2005ie}  denoted as fit III.

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.1]{chapter1-ris3}
\caption{Estimated Boer-Mulders asymmetries for NICA conditions.}
\label{fig:theor-boer}
\end{center}
\end{figure}

Also the predictions on Boer-Mulders asymmetries are given in Figure \ref{fig:theor-boer}.

The measurability of the asymmetries shown in above mentioned figures will be discussed in Section 7.

At the moment, only the COMPASS collaboration has presented the first experimental results on measurements
of Drell-Yang processes using a polarized \cite{compass:dy}. The measurement of transverse--spin--dependent 
azimuthal asymmetries in  Drell--Yan (DY) processes was performed by COMPASS collaboration using CERN SPS 
190 GeV/c $\pi$ − beam and a transversely polarized ammonia target. Three azimuthal asymmetries (TSAs) giving
access to different transverse--momentum--dependent (TMD) parton distribution functions (PDFs) are extracted
from experimental data Figure \ref{fig:compass-dy1}.  

\begin{figure}[h]
\begin{center}
\includegraphics[scale=1]{chapter1-ris5}
\caption{Extracted Drell--Yan TSAs related to Sivers, transversity and pretzelosity TMD PDFs (top to bottom).}
\label{fig:compass-dy1}
\end{center}
\end{figure}

The observed indication on sign change  in Sivers asymmetries is found to be consistent with the fundamental
prediction of QCD that the Sivers TMD PDFs extracted from DY have a sign opposite to the one extracted from
SIDIS data Figure \ref{fig:compass-dy2}.  Also two asymmetries originating from the pion Boer-Mulders TMD PDFs  were 
measured.

\begin{figure}[h]
\begin{center}
\includegraphics[scale=1]{chapter1-ris4}
\caption{The measured mean Sivers asymmetry and the theoretical predictions for different 
$Q^2$ evolution schemes. The dark-shaded (light--shaded) predictions are evaluated with 
(without) the sign--change hypothesis. }
\label{fig:compass-dy2}
\end{center}
\end{figure}


==> tex/case_PP.tex <==
\subsection{Prompt photon production}
As it was already mentioned in the Sec. , the two hard processes determine the production of prompt photons: gluon Compton scattering  $g q (\bar{q}) \to \gamma q (\bar{q})$ and quark-antiquark annihilation: $q\bar{q}\to g \gamma$. Contribution of the latter process to the total cross section does not exceed 20\% at the discussed energy range. 

%В лидирующем порядке теории возмущений в рождение одиночных прямых фотонов дают вклад два жёстких процесса: уже упомянутое выше глюонное комптоновское рассеяние $g q (\bar{q}) \to \gamma q (\bar{q})$ и кварк-антикварковая аннигиляция $q\bar{q}\to g \gamma$. Сечения этих процессов  как функции энергии в системе центра масс сталкивающихся протонов $\sqrt{s}$ для поперечного импульса фотонов $p_T>1$ ГэВ/с представлены на Рис. \ref{kinematic}(а) для набора функций партонных распределений протона NNPDF2.3. Именно доминирование процесса глюонного комптоновского рассеяния и определяет возможность использования прямых фотонов в качестве инструмента для изучения свойств глюонной компоненты протона. 




Prompt photons are photons that are produced by hard scattering of partons. According to the factorization theorem, the inclusive cross section for the production of a prompt photon in a collision of hadrons $h_A$ and $h_B$ can be written as follows:
\begin{equation}
d\sigma_{AB\to \gamma X}=d\sigma_{dir}+d\sigma_{frag}=
\sum_{a,b=q,\bar{q},g}\int{dx_a dx_b}f_a^A(x_a,Q^2)f_b^B(x_b,\mu^2)d\sigma_{ab\to \gamma x}(x_a, x_b, Q^2)+d\sigma_{frag}.
\end{equation}
Here, $d\sigma_{dir}$ is the contribution of photons emitted via direct coupling to a quark (direct photons) and $d\sigma_{frag}$ represents the contribution of photons produced from the fragmentation of a final partonic state (fragmentation photons). The function $f_a^A$ ($f_b^B$) is the parton density for hadron $h_A$ ($h_B$), $x_a$ ($x_b$) is the fraction of the momentum of hadron $h_A$ ($h_B$) carried by parton $a$ ($b$) and $Q^2$ is  the square of the 4-momentum transferred in the hard scattering process, and $\sigma_{ab\to \gamma x}(x_a, x_b, Q^2)$ represents the cross section for the hard scattering of partons $a$ and $b$. 
%The contribution of fragmentation photons does not exceed 10 -- 20\% in the discussed kinematic range, even for much higher energies \cite{Hanks:2009fj} and can be taken into account.
Prompt photon production in hadron collisions is the most direct way to access the gluon structure of hadrons. 

There are two main hard processes for the production of direct photons: i) gluon Compton scattering, $gq(\bar{q})\rightarrow \gamma q(\bar{q})$, which dominates, and ii) quark-antiquark annihilation, $q \bar{q} \rightarrow \gamma g$. Contribution of the latter process to the total cross section does not exceed 20\% at CMS energy $\sim 20$ GeV/c$^2$. 

\begin{figure}[ht]
\begin{center}
\includegraphics[width=0.8\linewidth]{fig05lnpp}
\caption{Measured cross sections of prompt-photon production divided to the predicted those by theory as function of  $x_T$ \cite{Aurenche:2006vj}.}
\label{fig:pp_prompt_unpolarized}
\end{center}
\end{figure}

Unpolarised measurements of the differential cross section of prompt-photon production 
in proton-proton(antiproton) collisions were already performed by the fixed-target and collider experiments. Figure \ref{fig:pp_prompt_unpolarized} shows the the ratio of the measured cross sections to the predicted by theory as function of  $x_T={2p_t}\sqrt{s}$ \cite{Aurenche:2006vj}. One can see that for the fixed-target results corresponding $\sqrt{s}\sim 20$ GeV there is significant disagreement with theoretical expectations that is absent for the high-energy collider results. A new precise measurement could clarify the problem.

The measurement of single transverse spin asymmetry $A^{\gamma}_N$ in prompt-photon production at high $p_T$ in polarised p-p and d-d collisions could provide information on the gluon Sivers function which is almost unknown at the moment \cite{Boer:2015vso}. The numerator of $A^{\gamma}_N$ can be expressed as \cite{Schmidt:2005gv}
\begin{eqnarray}
\nonumber
\sigma^{\uparrow}-\sigma^{\downarrow} &=&\sum \limits_{i}\int_{x_{min}}^1  dx_a \int
d^2{\bf k}_{Ta} d^2{\bf k}_{Tb}
\frac{x_a x_b}{x_a - (p_T/\sqrt{s})~e^y}
\left [ q_i(x_a,{\bf k}_{Ta}) \Delta_N G(x_b,{\bf k}_{Tb}) \right. \\
& & \times \frac{d\hat{\sigma}}{d \hat{t}}
 (q_i G \to q_i \gamma )
 +  \left.  G(x_a,{\bf k}_{Ta}) \Delta_N q_i (x_b,{\bf k}_{Tb})
 \frac{d\hat{\sigma}}{d \hat{t}} ( G q_i \to q_i \gamma  ) \right ]~~.
\end{eqnarray}
Here $\sigma^{\uparrow}$ and $\sigma^{\downarrow}$ are the cross sections of the direct photon production for the opposite transverse polarizations of one of the colliding protons,  $q_i(x,{\bf k}_{Ta})$ $[G(x,{\bf k}_{Ta})]$ is the quark [gluon] distribution function with specified ${\bf k}_{T}$ and $\Delta_N G(x_b,{\bf k}_{Tb})$ $[\Delta_N q_i (x_b,{\bf k}_{Tb})]$ is the gluon [quark] Sivers function. $d\hat{\sigma}/d \hat{t}$ represents corresponding gluon Compton scattering cross section. The authors of the work \cite{Qiu:1991wg} pointed out that the asymmetry $A^{\gamma}_N$ at large positive $x_F$ is dominated by quark-gluon correlations while at large negative $x_F$ it is dominated by pure gluon-gluon correlations as it was concluded in \cite{Ji:1992eu}. The further development of the corresponding formalism can be found in \cite{Hammon:1998gb,Gamberg:2012iq}. It is important to notice that the corresponding known non-zero asymmetry in $\pi^0$ production, $A^{\pi^0}_N$ [],  could be controlled in parallel.

The first attempt to measure $A^{\gamma}_N$ at $\sqrt{s}=19.4$ GeV was performed in the fixed target experiment E704 at Fermilab in the kinematic range $-0.15<x_F<0.15$ and 2.5 GeV/$c$ $<p_T<$ 3.1 GeV/$c$. The results were consistent with zero within large statistical and systematic uncertainties \cite{Adams:1995gg}. 

\begin{figure}[h]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{PP_pred_1} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{PP_pred_2} \\ (b)}
  \end{minipage}
  \caption{Theoretical predictions for $A^{\gamma}_N$ at $\sqrt{s}=30$ GeV and $p_T=4$ GeV/$c$ for (a) positive \cite{Hammon:1998gb} and (b) negative \cite{Qiu:1991wg} values of $x_F$.}
  \label{fig:pp_AN_theory}  
\end{figure}

     The study of prompt-photon production at large transverse momentum with longitudinally polarised proton beams could provide the access to gluon polarisation $\Delta{g}$ via the measurement of longitudinal double spin asymmetry $A^{\gamma}_{LL}$ \cite{Cheng:1989hf}. Assuming dominance of the gluon Compton scattering process, the asymmetry $A_{LL}^{\gamma}$ can be presented as \cite{Bunce:2000uv}

\begin{equation} \label{eqqg}
A_{LL} \approx \frac{\Delta g(x_a)}{g(x_a)} \, \cdot \, 
\Bigg[\frac{\sum_q e_q^2 \left[ \Delta q (x_b) + 
\Delta \bar{q} (x_b) \right]}{\sum_q e_q^2 \left[q (x_b)+
\bar{q} (x_b) \right] } \Bigg] \, \cdot \, 
\hat{a}_{LL}(gq \rightarrow \gamma q) + (a\leftrightarrow b) \, .
\end{equation} 
The second factor in the equation coincides, to lowest 
order with the spin asymmetry $A_1^p$ well-known from polarised DIS, 
and the partonic asymmetry $\hat{a}_{LL}$ is calculable in perturbative QCD. Previous results for gluon polarisation show that gluon polarisation is consistent with zero: $|\Delta{g}/g|<\pm0.2$ while the asymmetry $A_1^p$ is about 0.2. So. it seems, the value of $A^{\gamma}_{LL}$ should not exceed level of a few per cent. Measurement of $A_{LL}^{\gamma}$ asymmetry as well as $A^{\gamma}_N$ is the part of the spin physics programme at the RHIC collider \cite{JalilianMarian:2000qa},\cite{Sakashita:2009nba},\cite{Horaguchi:2006zz},\cite{Skoro:1999rg},\cite{doi:10.1146/annurev.nucl.50.1.525}.

Authors of the works \cite{Li:2008ym,Lansberg:2015hla} propose to pay attention to associative prompt-photon production in reactions like $p p \to \gamma J/\psi X$.

==> tex/case_gen.tex <==
\subsection{Studies of Non-Perturbative Quantum Chromodynamics via structure of
 hadrons and light nuclei }

Quantum Chromodynamics (QCD) is the only part of Standard Model which exhibits fully non-perturbative
 (NP) behaviour. In this respect it is similar to the rich and complicated phenomena  in condensed matter
 physics, hydrodynamics, plasma physics, astrophysics etc. 

The important information on NPQCD is provided by its phase diagram and various collective phenomena  
 emerging in heavy-ion collisions, which will be studied at BM@N and MPD detectors.

SPD will concentrate on the complementary way of NPQCD investigations which is provided by the exploration of hadron structure. In 
modern terms, the latter is described by the vast set of various parton distributions and correlations. The most
 general of them is ("mother") Wigner function, containing the full information about the longitudinal and
 transverse spin and momentum partonic degrees of freedom. The average over some variables or putting  
some other to particular (zero) values is leading to more simple and more easily measurable
description of fundamental particles, quarks and gluons, inside hadrons. The important stage of this
reduced
description consists of the set of Transverse-Momentum-Dependent Parton Distributions (TMDs) and the
 reduction process is finishing when most familiar collinear parton distributions appear.

SPD provides the unique opportunity of studies of various elements of NPQCD hadron structure in the
 same experiment. It opens the possibility of comparative studies of observables (especially the spin
 effects) in collisions of hadrons and light nuclei, which, in turn, may be compared to the data on heavy-ion
 collisions from MPD and BM@N.  It can also  reach complementarity between studies of tht same
 functions in lepton-hadron and hadron-hadron process, making use of similarity of kinematics of MPD with
 COMPASS and, partially, JLab. The core of this investigations is formed by the studies of spin-dependent and spin-independent TMDs. 

Usually the exploration of Parton Distributions is based on some sort of Factorisation Theorem (which in
 various cases is proved with different rigour) when the short-distance part of the process described by
 PQCD utilising the Asymptotic Freedom is used as a sort of "microscope" to probe the non-perturbative
 ones.  SPD will use several such microscopes. 

The most clean process is the production of massive lepton pairs discovered by Drell and Yan (DY) and, 
independently, at JINR, by Matveev, Muradyan  and Tavkhelidze (MMT). MMT-DY process with one transverse  polarized hadron allows one to measure the full set of leading TMDs. 

The measurement of TMDs requires to measure the angular distribution of lepton pair in its c.m. frame which  is related to the tensor polarization of virtual photon. It is of major importance even in unpolarized collisions,  being the probe of various aspects of hadron structure, including T-odd Boer-Mulders function, via the deviation from the  so-called Lam-Tung relation. 

The average over the transverse momentum of MMT-DY pair provides the probe of twist-3 ETQS quark-gluon correlators discovered in JINR by Efremov and Teryaev (fermionic poles) and by Qiu and Sterman (gluonic poles). The transverse twist-3 asymmetry in MMT-DY process  allows one to measure the gluonic pole correlator and test its normalization, which receives extra factor 2 from delicate QCD effect discovered recently in JINR. 

The MMT-DY process with polarized deuteron beam allows one to measure the tensor parton distribution which is related to the quark gravitational form factor.  These form factors got recently much attention due to the measurement  of pressure in proton. 

The production of exclusive MMT-DY pairs provide an access to another important objects - Generalized Parton Distributions, in particular to the ones related to the recently measured pressure of quarks in proton. 

Another process sensitive to TMDs ("microscope")  is $J/\Psi$ production. In the case of $q \bar q$ anihilation there is a duality to MMT-DY process (known also as fusion model) so that $J/\Psi$ dilepton decay plays the same role as MMT-DY itself, with accordingly increased statistics. 

Yet another process, sensitive to TMDs is direct photon production. 
It provides the direct access to various gluon TMDs.

The production of hadrons with large transverse momentum, contrary to MMT-DY and direct photon production,  is related to the necessity of taking into account the fragmentation process. At the same time, the increased  cross sections allow one the more accurate measurements. Such accurate measurements of transverse single spin asymmetries with varying rapidity and transverse momentum will make possible the scan of twist-3 correlators. This scan  may be combined with the similar studies in lepton-hadron scattering at COMPASS and JLab.

Large transverse momentum production also allows one to search for multiquark and exotic states, as well as consider probes of cold nuclear matter complementary to the search of short range correlations at BM@N.  

While SPD main target are hadronic collisions, the ultraperipheral nuclear ones may be also accessible.
In the nuclear-proton collisions such object as Wigner function may be measured.  


To summarize, SPD physical program is aimed to the measurement of various NPQCd functions, describing theproton structure. The main features of the program are:
\begin{itemize}
\item measurement of various TMDs in the same experiment;
\item  comparison of results for hadronic and light nuclear collisions which may be combined with MPD data for heavy-ion collisions;
\item complementarity to the lepton-hadron measurements.
\end{itemize}

==> tex/high_pt.tex <==
\subsection{Phenomena with high-p$_t$ hadrons}
The unique features of the SPD detector like:
\begin{itemize}
\item about full solid angle  $\Delta\Omega \sim4\pi$; 
\item registration of all kinds of particles; 
\item working at luminosity  $\geq 10^{30}$ cm$^{-2}$ s$^{-1}$; 
\item PID – close to full energy range and high momentum resolution;
\item working with polarized and nonpolarized  light nuclear beams;
\item the presence of tagging stations to detect spectator neutrons and protons which will allow to investigate the full set of isotopic states of nucleon-nucleon interactions ($p-p$, $p-n$ and $n-n$) in the polarization mode
\end{itemize}
allow to plan unique research program in the energy range of $\sqrt{s}$ from 3~GeV to 7~GeV.  In the area of high many phenomena had been discovered that have not been explained until now. These phenomena are continue manifesting in higher energy range but only in this energy can been providing the research of exclusive reactions and all type correlations for the rare processes. In higher energy range will be possible to provide investigations in semi-exclusive and inclusive reactions where some part of information will be lost.
	What key problems can be solved or obtained unique information that will give significant progress in the understanding of phenomena and development of their theoretical models? Significant progress can be made in the following issues:
\begin{itemize}	
\item  to define diquark properties which are crucial to describe huge the high $p_T$ baryon matter production and is a key stone for the exotic multiquark states explanation;
\item  to receive unique data about hadronization mechanisms;
\item  to expand experimental data (investigate full set of the isotopic nucleon-nucleon interactions) about the huge spin effects in the high $p_T$ region and try to define the nature of these effects;
\item  to provide more deep investigation of deuteron spin structure at the short distances;
\item  to investigate effect FSI especially with the strange hadrons ($NK$, $N\Lambda$ and s.o.) and to try detect the lightest hypernuclear  ($p\Lambda$) so very important issue for  definition of the EOS matter inside the massive stars;
\item  to define properties of Cold superDense Baryonic Matter (CsDBM) which is respond for the cumulative processes and may be have linked with states of nuclear matter at the core of the massive stars too;
\item  to provide detail investigation of hyperon polarization in the high $p_T$  region and resolve nature of this effect;  
\item  to look at the nature of the dilepton production anomaly in np(may be nn) collisions;
 \item  to find direct production of the exotic multiquark states as pentaquark and the tetraquark especially
       in the light quark sector;
\item to define mechanism of subthreshold $J/\psi$ production.
\end{itemize}

\begin{figure}[h]
  \begin{minipage}[ht]{0.55\linewidth}
    \center{\includegraphics[width=1\linewidth]{hpt_1} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.43\linewidth}
    \center{\includegraphics[width=1\linewidth]{hpt_2} \\ (b)}
  \end{minipage}
  \caption{(a) Momentum spectrum of particles emitted at 90$^{\circ}$ from a
beryllium target struck by 30 Bev protons. The ordinate is the
number of particles produced at the target per steradian per Bev/$c$
per circulating proton. The dashed portions of the curves indicate
regions where the corrections due to multiple scattering exceed
15\%. At the time these data were taken no effort was made to
detect He$^3$. (b) Ratio deuterons/protons as a function of momentum
for particles emitted a) at $\Theta_{LS}=15.9^{\circ}$ \cite{Cocconi:1960zz}; b) at $\Theta_{CMS}\sim90^{\circ}$ \cite{Abramov:1986ti}.
}
  \label{fig:hpt1}  
\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.8\linewidth]{hpt_4}
\caption{Proton-proton elastic cross section for $\Theta_{CMS}\sim90^{\circ}$ [6]. }
\label{fig:hpt4}
\end{center}
\end{figure}

\subsubsection{	The phenomena with unpolarized beams which not understand up to now}
The particle production in the high $p_T > 1$ GeV/$c$ region began to study with the beginning in operation of the PS (CERN) and AGS (BNL) accelerators. The first measurements of the particle yield at angles close to 90$^{\circ}$ in c.m.s. showed a significant increase yield of nucleons and nuclear fragments compared with the mesons \cite{Cocconi:1960zz,Fitch:1962fq,Schwarzschild:1963zz}.The Fig. \ref{fig:hpt1}(a) shows the data from \cite{Fitch:1962fq} for particles and nuclear fragments that were emitted at an angle of 90$^{\circ}$ in the laboratory system. It is important to emphasize that these measurements were the first when the data were simultaneously obtained in the kinematics of nucleon-nucleon interaction and out off this kinematical border, in the so-called cumulative region, when several nucleons must participate in the interaction as a single object. They most vividly illustrate the riddle that had arisen – an absolute dominance of the baryonic matter (nucleons and nuclear fragments) in the cumulative high $p_T$ region. 60th years didn’t bring the complete understanding of the nature of this phenomenon.
Studies of the 70--90s of the last century at higher proton energies not only confirmed the previously observed effects but also had raised the question of the range of applicability of the plain parton model, which predicted the dominance of mesons in the high $p_T$ region. The investigations were carried out on the Tevatron (FNAL) up to the proton beam energy 800 GeV \cite{Cronin:1974zm} and with proton beams in the Institute of High-Energy Physics (Protvino) on the accelerator U-70 with energy up to 70 GeV \cite{Abramov:1985ct,Abramov:1986ti,Sulyaev:1989ze}. The real challenge for the parton model had become the observation of a constant in ratio deuterons/protons as in pp- so pA-collisions in the range of transverse momenta from 1 to 4 GeV/$c$. The Fig. \ref{fig:hpt1}(b) shows data from \cite{Cocconi:1960zz} at proton energy 25 GeV and at proton energy 70 GeV \cite{Abramov:1986ti}. Investigation of the energy dependence of the elastic cross section of the p-p scattering at an angle 90$^{\circ}$ cms also led to an unexpected result \cite{Akerlof:1967zz}. In this work for the first time was obtained "dynamic" confirmation of the hypothesis of quarks or other words composite nature of hadrons, which was appeared not long before in 1964. The Fig. \ref{fig:hpt4} shows the data of the work \cite{Akerlof:1967zz}. On the presented graph there is a sharp kink in the cross section in the  $\sim$4 GeV region.

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.8\linewidth]{hpt_5}
\caption{The puzzles of the spin phenomena not resolve up to now. }
\label{fig:hpt5}
\end{center}
\end{figure}

\subsubsection{The polarized beam puzzles}
The further studies of the elastic p-p scattering in the region of high $p_T$ with polarized proton beams and a polarized target had confirmed that the nature of strong interaction changes drastically in this  $\sim$4 GeV energy region \cite{OFallon:1977fkf,Crabb:1978km,Lin:1978xu,Crosbie:1980tb}. It was discovered huge polarized effects which contradict with the QCD predictions \cite{Krisch:2007zza}. The summary of the effects which haven’t theoretical explanations is presented at Fig. \ref{fig:hpt5}. where included figures from  \cite{Krisch:2007zza} and \cite{Crabb:1979nh}. Now there is only one data for double spin elastic np-scattering \cite{Crabb:1979nh} at $p_{LAB}=6$ GeV/$c$ which stress the importance to provide investigation for full set of isotopic states for nucleon-nucleon interaction.   


==> tex/jpsi.tex <==
\subsection{Charmonia production}
The $J/\psi$ (and charmonia in general) production in hadron
collisions is of great interest
for several reasons. Firstly, the description of the process
is a challenge and an important test for our
understanding of QCD. Despite of considerable efforts
that have been devoted to study of the charmonia production
since the $J/\psi$ discovery and existence of several theoretical
approaches to the problem, no fully consistent understanding of the process
has been obtained yet.
Secondly, comprehensive understanding of the charmonia production process
would allow one to separation of quark-antiquark
annihilation and gluon-gluon fusion contributions, and thus
to benefit from large (compared to the Drell-Yann process) statistics
of inclusive $J/\psi$ events to measure and interpret
transverse spin asymmetries. 
Thirdly, the production process is sensitive to gluon content of
of colliding hadrons, while experimentally $J/\psi$ can be easily
reconstructed from the very clean dilepton modes, making it
a powerful tool to probe gluon parton distribution functions (PDF).
Its is of special interest for pion and kaon, since the gluon
PDF of the former is poorly know and gluon PDF of the latter
has not been measured yet.
In fact, inclusive $J/\psi$ production is one out of two
available experimental methods (along with prompt photons) to probe
these gluon distributions in the current and foreseen experiments
with pion and kaon beams []. It must be noted, that
a significant fractions (about 40\%) of $J/\psi$ mesons are produced
indirectly through decays of of $\chi_{cJ}$ and $\psi(3686)$ (so called
feed-down contributions),
thus requiring dedicated study of these charmonium states.
%Reliable extraction of gluon PDF of pion and kaon
%is model dependent and relies on understanding of the charmonia
%production process.
All experimental applications of the charmonia production
rely on our theoretical understanding of the process.
The SPD experiment might be ideal tool to verify and validate theoretical
approaches at relatively low energies and to obtain related physical results.
\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{fig/nrqcd_cem}
\includegraphics[width=0.8\textwidth]{fig/nrqcd_cem2}
\caption{\label{fig:nrqcd-cem} NRQCD (left column) and CEM (right column) predictions for $d\sigma/dx_F$ from Ref.~\cite{Vogt:1999dw} showing
contribution from the gluon-gluon fusion (the dashed line) and quark-antiquark annihilation (the dash-and-dotted line) for
center-of-mass energies of 15~GeV (top) and 39~GeV (bottom)}
\end{figure}
Reviews on charmonia production mechanisms can be found in Ref.~\cite{Brambilla:2010cs, Brambilla:2014jmp}.
Describing models relevant for SPD collision energies it is worth
to start from the color-singlet model (CSM). In this
model the charmonia resonances are formed from $c\bar{c}$ pair produced
in the color singlet state with the angular momentum and spin alignment
corresponding to quantum numbers of the produced state.
The hadronization of the $c\bar{c}$ can be related to decays
of charmonia states
or to values or derivatives of heavy quark wave function in
the charmonium potential models. However, this model systematically
underpredicts charemonia production rate. The most notable example
is $\psi(3686)$ production at Tevatron underestimeted by factor of 30 %(?)
at LO. Despite the later calculation show that the next to the
leading order (NLO) calculations substantially
increase the cross-section [], the model still significantly underestimates
the cross-section in this and many other cases.
The two contemporary used approaches are the color evaporation model (CEM)
and non-relativistic QCD (NRQCD), which are usually formulated for collinear
factorization of hadron scattering. In both models formation
of charmonia state is also possible from the color-octet configuration
of a $c\bar c$ pair, which becomes color neutral during formation
of a charmonium state by soft interaction with the collision-induced
color field. In CEM charmonium state production cross-section is
assumed to be proportional to production cross-section of
$c\bar c$ pair with the invariant mass between $2m_c$, where
$m_c$ is the mass of $c$-quark, and open charm threshold.
For explicit formulas see e.g. Ref.~\cite{Vogt:1999dw}.
In this model the sum over colors and spins of the $c$ and $\bar c$
quarks is implied. The proportionality coefficients for given charmonium
state are assumed to be process independent
(comparison to experimental data shows that it hold only to some extent~\cite{Bodwin:2005hm}).
Despite of its simplicity, this phenomenological model it provides
reasonably good descriptions of $\sqrt{s}$-dependence, $d\sigma/dx_F$
($x_F$ is the ratio of the $J/\psi$ longitudinal momentum to its
maximal value the reaction center-of-mass reference frame) \cite{Gavai:1994in}.
If the NLO terms
are taken into account, it also predicts $J/\psi$ transverse
momentum distribution ($p_T$), but results require $k_T$ smearing
for more or less reasonable data description at high energies~\cite{Bodwin:2005hm}.
The nonrelativistic QCD is the most rigorous approach to
charmonia production (the very details of the approach can be
found in Ref.~\cite{Bodwin:1994jh}). It is based on two points.
The first point is factorization conjecture that assumes that
the parton cross-section
factorizes to hard perturbative part that describes production of
$c\bar c$ pair on the scale of $1/m_c$ and nonperturbative soft
part that describes formation of charmonia state:
\begin{equation}
\label{eq:nrqcd}
\hat\sigma(ij\to H + X) = \sum_n C^{ij}_{n} \langle O^{H}_n \rangle .
%\[ \sigma_H = \sum_{i,j} \int_0^1 dx_1 dx_2 f_{i/A}(x_1)f_{i/B}(x_2)\hat\sigma(ij\to H).
\end{equation}
Here indexes $i$ and $j$ denote interacting partons, $H$ and $X$ state for
charmonia state and rest of produced particles, the sort-distance
coefficients (SDC) $C^{ij}_{n}$ describe production of a $c\bar c$ pair
in the state $n$ ($n$ denotes relative momentum, spin alignment and
color state), and, finally, the long-distance matrix elements (LDME)
$\langle O^{H}_n \rangle$ describe hadronization of the $c\bar c$ pair
to charmonia state $H$. It is important to stress that this conjecture
is proven only for specific cases []. An important consequence of these
factorization is the process independence fo LDME (e.g. in hadron
collisions, photoproduction, $e^+e^-$ annihilation).
The second point is that there is a hierarchy of LDME $\langle O^H_n \rangle$
with respect to $v$ ($v^2\sim0.2-0.3$) -- typical velocity of heavy quark in
the charmonium  system. Thus, Eq.~\ref{eq:nrqcd} is a double series in $\alpha_S$ and $v^2$.
Both of these parameters are of order of 0.2-0.3, which may rise concerns
about convergence of the series. The color-singlet LDME are obtained
in the same way as in CSM. The color-octet LDME are obtained from fits
to the data or lattice calculations (the latter available only for 
$\chi_{cJ}$ \cite{Bodwin:1996tg}). Verification of the LDME universality
in different $J/\psi$ production processes) is one of the direct tests of
NRQCD. The Ref.~\cite{Butenschoen:2012qr} reviews NLO NRQCD fits to different
data sets, that include $p_T$ distribution in proton-proton collisions (ATLAS, CDF),
the same distribution in photoproduction at H1, polarization data (CDF)
and $J/\psi$ production in $e^+e^-$
annihilation at Belle showing that all available data sets can not be
described simultaneously by one set of LDME.
That may have several explanations including limited applicability of
NRQCD, failure of fixed-order QCD expansion for SDC, slow convergence of
NRQCD $v$-expansion or inclusion $d\sigma/dp_T$ data for small
small $p_T$. The latter differential cross-section is not described
by NRQCD LO and NLO formulas because of increasing role
of soft gluon emission and  non-negligible $k_T$ of partons.
The typical low $p_T$ cut-off value for NRQCD fits is around
3--5~GeV, much larger than typical $J/\psi$ transverse momenta at SPD.
Here $k_T$ factorization approaches might become a better options,
as they take into account $k_T$ dependence of PDF and ``partially'' take
into account soft gluon emission through PDF evolution equations \cite{Brambilla:2014jmp}. %??

The description of the  differential cross-section with respect to $x_F$
is one the direct tests of charmomia prodcution at SPD energies.
Previously, it was used by NA3 to separate the gluon-gluon fusion and
quark-antiquark annihilation~\cite{Badier:1983dg} as well as by E537
to probe gluon distributions of pion~\cite{Tzamarias:1990ij}.
The Ref.~\cite{Vogt:1999dw} gives prediction of CEM and
NRQCD models for collision energies of 15~GeV and 39~GeV. The
total line shape and relative
contributions of the gluon-gluon fusion and
quark-antiquark annihilation are shown in Fig.~\ref{fig:nrqcd-cem}.

\begin{figure}[h]
\centering
\includegraphics[width=0.8\textwidth]{Jpsi_sections_NRQCD_SPD}
\caption{\label{fig:nrqcd-data_spd} Experimental data for the $J/\psi$ production cross section and the NRQCD fit result \cite{Maltoni:2006yp}. The SPD energy range is shown in red.}
\end{figure}

The SPD experiment at NICA could provide precise measurements
of total cross-section, differential cross-sections with respect to $x_F$ and
$p_T$ and polarization for $J/\psi$. The open geometry of the SPD detector
may allow measurements of same observables for $\psi'$, $\chi_{c1}$
and $\chi_{c2}$, which were not possible in the set-up of the previous
fixed-target experiments with the same interaction energy. It must be noted,
that analysis of the $\psi'$ production would be much simplified
due to the absence of the feed-down contribution.
The existing experimental data for the total cross section of the $J/\psi$ production in the proton-nucleon collisions fro different energies are presented in the Fig. \ref{fig:nrqcd-data_spd} together with the NRQCD fit. The SPD experiment will cover the most interesting range where on the one hand there is discrepancy between the experimental results and on the other hand the NRCSD prediction fits data  insufficiently.

\subsubsection{TMD PDFs in $J/\psi$ production}

The production of lepton pairs in the $q\bar{q}$ annihilation processes, via the $J/\psi$ production and its subsequent decay is analogous to the Drell-Yan production mechanism. The analogy is correct if the $J/\psi$ interactions with quarks and leptons are of the vector type. This analogy is known as the duality model \cite{Anselmino:2004ki,Leader:1982gt}. For the TMD PDF
studies, the duality model can predict \cite{Barone:2006ws} a similar behavior of the azimuthal asymmetries in the
lepton pair's production via Drell-Yan  and via the $J/\psi$ leptonic decay This similarity follows from the idea of the duality model to replace the coupling $e_q^2$ by the $J/\psi$ vector coupling with $q\bar{q}$ $(g_q^V)^2$
 The vector couplings are expected to be the
 same for $u$ and $d$ quarks \cite{Anselmino:2004ki} and cancel out in the azimuthal asymmetries for large values of $x_1$ or $x_2$. 
 For instance we can compare the Sivers asymmetry for Drell-Yan with the corresponding asymmetry for  $J/\psi$ events 
 at different colliding beam energies.

\input{xyz}

==> tex/nica_gpds11.tex <==
\subsection{Generalized parton distributions}
There are several ways to study Generalized Parton Distributions (GPDs), which are important complementary ingredients of hadron structure, at NICA 
%\section{GPDs in vector  meson production.}
The NICA detector should have a detailed determination of the
final particles. In this case it is possible to detect an
exclusive reactions like $pp \to pp M$ where $M$ is a some meson.
The reaction when the proton radiate a 
%hard 
photon with small virtuality
which interact with the other proton and produce the meson
$M$ is shown in Fig. \ref{fig:gpd1}(a).  In the final state we should
observe meson $M$ and two protons. 
%The virtuality $Q^2$ can be
%determined from the final proton angle and momenta. 
%We shall see
%later that 
and in addition to photon in the vector meson (VM)
production the odderon exchange is possible.

\begin{figure}[h]
  \begin{minipage}[ht]{0.42\linewidth}
    \center{\includegraphics[width=1\linewidth]{fig01} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.56\linewidth}
    \center{\includegraphics[width=1\linewidth]{golf7aa} \\ (b)}
  \end{minipage}
  \caption{(a) Vector meson production at NICA via photoproduction mechanism or odderon exchange.
  (b) Drell-Yan process with gluon and quark GPDs.
  \label{fig:gpd1}}
\end{figure}

%\begin{figure}[h]
%\epsfxsize=5.5cm \centerline{\epsfbox{fig01.eps}}
%\caption{\label{f1} Vector meson production at NICA via
%photoproduction mechanism or odderon exchange}
%\end{figure}


At NICA we shall have the energy in the $\gamma p$ system
$W=\sqrt{s_2=(q+p)^2} \sim 5-15~\mbox{GeV}$.  
%At large  $Q^2$ 
The
meson photoproduction amplitude can be presented in a factorized
form as a convolution of the hard scattering part which can be
calculated perturbatively and the Generalized Parton Distributions
\cite{Goloskokov:2006hr,Goloskokov:2007nt}.

This photoproduction contribution is similar to the corresponding
process in lepton-proton reaction. However in the proton-proton
reaction we should have in addition to photon exchange the strong
interaction contribution. Estimations shows that at NICA the
energy $s_1=(p_1'+q')^2$ is rather large $s_1 \geq
100$ GeV$^2$. At such energies the gluon contribution should
predominate. The minimum number of gluons which can contribute to
the Vector Dominance (VD) production process is equal to 3. This exchange can be
associated with the odderon contribution. So we shall have at NICA
in VM production photon contribution and odderon effects, Fig. {fig:gpd1}(a).
The interference of these effects is of special interest.
Generally odderon can be effectively regarded as an object similar
to the photon. In this case the  odderon contribution will be
expressed in terms of GPDs as the photoproduction amplitude.

In the ultraperipheral processes one may also study the most general non-perturbative objects, 
Generalized Transverse Momentum dependent Distributions (GTMD). This possibilities was explored at high energies \cite{Hagiwara:2017fye} but may be also continued to lower energies
of NICA.

One may also consider the ultraperipheral collisions of protons with heavy ions in SPD,
which will enhance the photoproduction contribution by several orders of magnitude.  
%(R. Tsenov)

The $J/\psi$ production can be studied at $W \sim 15~\mbox{GeV}$
%and $Q^2 \sim 2 \mbox{GeV}^2$. 
Large meson mass permit to perform
perturbative calculation at sufficiently low $Q^2$. 
%At not very
%large $Q^2$  
and the photon exchange in $J/\psi$ production should
dominate. Cross section in the photon channel is about
$\sigma_{J/\psi} \sim 10 ~\mbox{nb}$. This process is dominated by
the gluon GPDs $H^g$. The $\tilde H^g$ effects determined by
$\Delta g$ can be tested in the $A_{LL}$ asymmetry of $J/\psi$
production.

%Note that that we have estimated cross section of light meson
%photoproduction  mechanism in \cite{sgv1}. Generally, this channel
%can be dominated in all the cases because the odderon contribution
%can be rather small in most reactions.

%\section{Exclusive Drell-Yan process with two GPDs contribution.}

The  exclusive Drell-Yan  production in the proton-proton
reaction determined by  two GPDs contribution was proposed in
\cite{Teryaev:2005uj}. This gives possibility to study GPDs at NICA within
the exclusive reaction  where in the final state we observe two
protons and the lepton pair. An example of such process that
contains gluon and quark contribution is shown in Fig. \ref{fig:gpd1}(b).


%\begin{figure}[h]
%\epsfxsize=7.7cm \centerline{\epsfbox{golf7aa.eps}}
%\caption{\label{f8}
% Drell-Yan process with gluon and quark GPDs }
%\end{figure}

 Investigation of the
cross section determined by two-GPDs effects is in progress now
\cite{Goloskokov:2018}.  It is shown that the gluon and quark sea GPDs lead to
the cross section which does not decrease with energy. Thus, this
reaction can be studied  at high energies. We estimate cross
section at NICA energies $\sqrt{s}=24~ \mbox{GeV}$ and $Q^2=5~
\mbox{(GeV/c)}^2$ integrated over $s_1$ and $s_2$.
 Preliminary results for  $d
\sigma/(d Q^2 d t_1 d t_2)$ -in~$\mbox{pb/(GeV/c}^6$ are shown in
Fig.\ref{fig:gpd2} as a function of momenta transfer $t_1$ and $t_2$.
The cross section of exclusive Drell-Yan process is equal to zero at
$t_1=0$, $t_2=0$. It has a strong maximum at rather small momentum
transfer and decrease exponentially at higher $t_1,t_2$. At
maximum cross section is about $40-50~\mbox{pb/(GeV/c)}^6$. Integrated
over $t_1,t_2$ Drell-Yan cross section $d \sigma/dQ^2 \sim 3~
\mbox{pb/(GeV/c)}^2$. This result is smaller with respect to the cross
section of inclusive Drell-Yan reaction because the contribution
Fig.\ref{fig:gpd1}(b)
 is a part of inclusive process. Estimations show that
such contribution is rather small but might be visible at NICA.
The $J/\psi$ mesons can be produced in a similar way.

\begin{figure}[h]
\begin{center}
  \begin{minipage}[ht]{0.56\linewidth}
   \includegraphics[width=1\linewidth]{ds2g}
  \end{minipage}
  \caption{Preliminary results for cross section of exclusive
Drell-Yan process over $t_1$ and $t_2$ at NICA energies and
$Q^2=5~\mbox{(GeV/c)}^2$.
  \label{fig:gpd2}}
\end{center}
\end{figure}
%\begin{figure}[h]
%\epsfxsize=10.5cm \centerline{\epsfbox{ds2g.eps}}
%\caption{\label{f3}
% Preliminary results for cross section of exclusive
%Drell-Yan process over $t_1$ and $t_2$ at NICA energies and
%$Q^2=5 \mbox{GeV}^2$.}
%\end{figure}

In the light $\rho,
\omega$ VM production we can test $H$, $\tilde H$, $E$ GPDs
contributions. $J/\psi$ production will give information about
gluon GPDs $H^g$, $\tilde H^g$. Exclusive Drell-Yan process with double
GPDs contribution is an important test of GPD model. Drell-Yan cross
section is rather small, but hopefully might be analysed.

Thus, important information on GPDs structure can be obtained at
NICA  with polarized beams.


==> tex/soft.tex <==
\section{Software design and computing}
\input{spdroot.tex}

==> tex/spdroot.tex <==
\subsection{SPDroot}
Monte Carlo simulation, event reconstruction for both simulated and real data, data analysis and visualization are planned to be performed 
by an object oriented C++ toolkit SPDroot. It is based on the FairRoot framework initially developed for the FAIR experiments at GSI Darmstadt and partially compatible with MPDroot and BM@Nroot software used at MPD and BM@N, respectively.

The SPD detector description for Monte Carlo simulation is based on the ROOT geometry while transportation of secondary particles through material of the setup and simulation of detector response is provided by GEANT4 code. The standard multipurpose generators like Pythia6 and Pythia8 as well as specialised generators can be used for simulation of primary nucleon-nucleon collision. An example of p-p collision event in the SPD detector visualised by the SPDroot event viewer is shown in Fig. \ref{fig:SPDroot}

\begin{figure}[!h]
    \center{\includegraphics[width=1\linewidth]{SPDroot}}
  \caption{Event viewer of the SPDroot.
 }
  \label{fig:SPDroot}  
\end{figure}

==> tex/timelines.tex <==
\chapter{Project timeline}
We propose a five-year project for delivering of a complete technical design of the SPD facility based on 
the necessary simulation work, prototypes construction and test measurements.\\

The timeline is seen like follows:

\begin {itemize}
\item Approval of a formal JINR project for design of the  SPD facility 
by the PAC for HEP in its meeting in January 2019;
\item 
Setting up of the SPD collaboration and election of its management bodies (2019);
\item  
Signing of MoU based on ''Regulations for the organization of experiments 
conducted by international collaborations using 
the capabilities of the JINR basic facilities'' \cite{rules}
% Please, insert here the following link: 
%http://www.jinr.ru/wp-content/uploads/JINR_Docs/Regulation_for_the_organization_of_experiments_eng.doc 
(2019);
\item Preparation of  Conceptual Design Report and its approval 
by the PAC for HEP at its meeting in January 2020;
\item Preparation of Technical Design Report for the first stage of the facility, including prototyping and test measurements (2020 -- 2022);
\item Preparation of Technical Design Report for the second stage (2023);
\end {itemize}

We hope to be able to start  construction of the first stage of the detector in 2022
 and perform first measurements somewhere in 2025.

